Binary Code Summarization: Benchmarking ChatGPT/GPT-4 and Other Large Language Models

Binary code summarization, while invaluable for understanding code semantics, is challenging due to its labor-intensive nature. This study delves into the potential of large language models (LLMs) for binary code comprehension. To this end, we present BinSum, a comprehensive benchmark and dataset of over 557K binary functions and introduce a novel method for prompt synthesis and optimization. To more accurately gauge LLM performance, we also propose a new semantic similarity metric that surpasses traditional exact-match approaches. Our extensive evaluation of prominent LLMs, including ChatGPT, GPT-4, Llama 2, and Code Llama, reveals 10 pivotal insights. This evaluation generates 4 billion inference tokens, incurred a total expense of 11,418 US dollars and 873 NVIDIA A100 GPU hours. Our findings highlight both the transformative potential of LLMs in this field and the challenges yet to be overcome.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.


==> figures/comment-parsing-challenge-old.tex <==
\begin{figure}[t]
%\raggedleft
\centering
\begin{minted}[mathescape,
               linenos,
               numbersep=5pt,
               %gobble=2,
               % frame=lines,
               frame=single,
               fontsize=\footnotesize,
               %fontsize=\footnotesize,
               %framesep=2mm,
               xleftmargin=10pt
               ]{c}
/* Return all but the first "n" matched 
  characters back to the input stream. */
#define yyless(n) \
    do \
    { \
        int yyless_macro_arg = (n); \
        YY_DO_BEFORE_ACTION; \
    } \
    while ( 0 )

/* yylex_destroy is for both reentrant 
    and non-reentrant scanners. */
#ifdef __cplusplus
static int 
yylex_destroy  (const char * yybytes, 
                int  _yybytes_len ) 
#else
static int 
destroy  (const char * yybytes, 
    int  _yybytes_len )
#endif
{
    /* Pop the buffer stack, 
        destroying each element. */
    while(YY_CURRENT_BUFFER){
        // Delete current buffer
        yy_delete_buffer( YY_CURRENT_BUFFER  );
        YY_CURRENT_BUFFER_LVALUE = NULL;
        yypop_buffer_state();
    }
    ...//skip for simplicity
    return 0;
}
\end{minted}
\caption{An Example of Various Developer-written Code Comments from Binutils-2.39. From line 13 to 21, the \texttt{ifdef} preprocessor directive is used to conditionally define a function with different names. For code comments, they are created for not only functions but also statements (e.g., line 26), basic blocks (e.g., lines 23 and 24), and the macro definition (lines 1 and 2).
\Xin{Change this example to a little simpler}}
% \vspace{-0.2in}
%Unintended concurrent enclave calls.}
\label{fig:comment-example}
\end{figure}

==> sections/background.tex <==

\subsection{Problem Definition}
\label{sec:definition}

\paragraph{Binary Code Summarization}
Given a binary executable $b\in \mathcal{B}$, the binary code $x\in \mathcal{X}$ are extracted and generated by binary analysis tools, which could be machine code, assembly code, intermediate representation (IR) code, or decompiled code.
% The binary analysis results $R$ are fed into the 
% Binary code summarization is to generate a description $Y$ by a semantic encoding function $\mathcal{}$
A binary code summarization system, \( \mathcal{M}: \mathcal{X} \rightarrow \mathcal{Y} \), generates a natural language summary \( y \in \mathcal{Y} \), capturing the semantic essence of the input context \( x \) and providing a high-level understanding of what a particular piece of code does.
\Xin{Move to overview section}


\ignore{
\paragraph{In-context Learning} 
% In-context learning~\cite{brown2020language} was initially proposed to generalize GPT-3 on out-of-domain tasks by learning context information from in-context instruction (aka zero-shot learning) or demonstration samples (aka few-shot learning).
The concept of in-context learning, as outlined in \cite{brown2020language}, was initially introduced to enhance the generalizability of GPT-3 for tasks beyond its primary domain. 
This is achieved by imparting the model with contextual knowledge through in-context instructions, which is commonly referred to as zero-shot learning, or through demonstration samples, a technique known as few-shot learning.
% Specifically, in-context learning involves adding a piece of system instruction $\mathcal{I}$ along with zero or $n$ in-context demonstration pairs ($\mathcal{X}_{d}$, $\mathcal{Y}_{d}$), where $\mathcal{X}_{d}$ and $\mathcal{Y}_{d}$ are sample inputs and outputs, before the test input:
To be more specific, in-context learning entails the inclusion of a system instruction $\mathcal{I}$ along with either 0 or $n$ in-context demonstration pairs ($\mathcal{X}_{d}$, $\mathcal{Y}_{d}$), where $\mathcal{X}_{d}$ and $\mathcal{Y}_{d}$ represent sample inputs and outputs. This augmentation occurs prior to the introduction of the test input:

\begin{equation}
    x = \{\mathcal{I}; (x_d^{i}, y_d^{i})_{0}^{n}; x_{t}\}
\end{equation}
\noindent where the system instruction and demonstration samples are concatenated with the test input $x_{t}$ to form the query input $x$.
\Xin{Move to section 4.2}
}

% \paragraph{Prompt Tuning}
% Although in-context learning has demonstrated great cross-task transferability, it still struggles to generalize on out-domain tasks. 
% To address such issues, prompt tuning was proposed to modify the input to LLMs without modifying the model parameters.
% Formally, the prompt tuning input can be expressed as:

% \begin{equation}
%     X_{PT} = \{E; X_{test}\}
% \end{equation}

% where $E = \{e_1, ..., e_m\}$ is the tunable prompt embeddings, which is encoded from the sequences of the demonstration inputs $X_{d}$ and the outputs $Y_d$.
% $X_d = \{x_1, ..., x_u\}$ and $Y_d = \{y_1, ..., y_v\}$ denote the sequences of input and output tokens.

\subsection{Background}
\label{sec:backgound}

\paragraph{Large Language Models} 
The widespread adoption of Large Language Models (LLMs) has been driven by significant advancements in various machine learning tasks~\cite{brown2020language}, such as machine translation and reading comprehension. 
These advances have enabled the scaling of LLMs to encompass billions of parameters and the utilization of billions of training samples.
LLMs are initially trained to incorporate knowledge across diverse domains, employing pretraining techniques such as mask token prediction and next sentence generation~\cite{devlin2018bert}. 
Subsequently, LLMs are applied to downstream tasks through either fine-tuning or prompting strategies~\cite{liu2023pre}.
Fine-tuning involves the process of updating model parameters by minimizing the loss on task-specific datasets, ultimately optimizing performance on these downstream tasks. 
However, it's worth noting that fine-tuning can be resource-intensive due to the necessity of weight updates and model training. 
This can pose challenges when sufficient training data, hardware resources, or access to LLMs themselves are not readily available.
Simultaneously, the approach of prompting entails directly executing model inference on LLMs without the need for training them on specific downstream task data. 
In order to provide LLMs with context, prompts are formulated using query examples and the desired generation results. 
This practice is commonly referred to as in-context learning as we defined in~\S\ref{sec:definition}, as it equips LLMs with the necessary contextual information for task execution.
% The widespread adoption of Large Language Models (LLMs) has been propelled by significant advances in various machine learning tasks, e.g., image classification and machine translation, enabling the scaling of LLM size to billions of parameters and utilization of billions of training samples.
% LLMs are trained to encompass knowledge from diverse domains based on the pretraining approaches, e.g., mask token prediction and next sentence generation.
% LLMs are then employed in downstream tasks through either fine-tuning or prompting approaches.
% Fine-tuning is a process of updating model parameters by minimizing the loss on task-specific dataset, rendering the optimal performance on downstream tasks.
% However, fine-tuning can be costly due to the need of weight updates and model training, which may not be feasible because of the unavailability of sufficient training datasets, hardware resources and no access to the LLMs themselves.
% Fine-tuning involves updating the model parameters using a specific training dataset to target a particular downstream task. However, fine-tuning can be costly due to the need for additional model training and may not be feasible when sufficient training datasets are unavailable. 
% Meanwhile, prompting involves directly execute model inference on LLMs without training them with downstream task data.
% To offer LLMs with in-context data, propmts are designed with examples of queries and generation results, which is often known as in-context learning or few-shot learning.
% On the other hand, prompting involves directly utilizing LLMs without any training by providing natural language descriptions of the downstream task and optionally offering a few task-solving demonstrations as input to the LLM.

\paragraph{Automated Code Summarization}
% Research in automated code summarization concerns the study
% of systems and methods for expressing code fragments
% (in most cases methods or functions) written in a given
% programming language with a natural language expression that
% % encapsulates their functionality or purpose. 
Automated code summarization aims at articulating code fragments, typically methods or functions, authored in a specific programming language, using natural language expressions that encapsulate their functionality or intended purpose~\cite{shi2022evaluation}.
% Recently, most of the works focus on source code summarization, inspired by natural language processing (NLP) approaches designed for text summarization, which in the last years are almost all based on neural
% architectures, and especially on transformer models
Lately, the predominant focus of this research has been on summarizing source code, inspired by natural language processing (NLP) techniques developed for text summarization~\cite{sharma2021survey}. 
Notably, in recent years, a substantial portion of these efforts has leaned heavily on neural architectures, with a particular emphasis on transformer models~\cite{guo2020graphcodebert,wang2021codet5,feng2020codebert}.
% Code summarization is the process of automatically generating concise and human-readable summaries or descriptions of code written in programming languages. 
% These summaries are intended to provide a high-level understanding of what a particular piece of code does, its functionality, and its purpose, without the need to read the entire codebase. 
% In the field of software engineering, this topic is of paramount interest due to its direct connection with the challenge of automating the generation of comments and documentation.
% Numerous endeavors have been undertaken in this area. 
% The majority of these studies~\cite{feng2020codebert,wang2021codet5,guo2020graphcodebert,ahmad2021unified,wang2022bridging} focus on generating summaries for small code blocks, such as individual methods. 
% This category also encompasses research on summarizing small code fragments~\cite{nazar2016source}, implementing code folding within integrated development environments~\cite{viuginov2019machine}, generating commit messages~\cite{liu2018neural,dong2022fira,liu2022commitbart}, and creating titles for online posts derived from code~\cite{du2019leopard}.
% To accomplish code summarization tasks, previous research endeavors have introduced three principal paradigms for modeling code semantics.
% As the first category, early works~\cite{haiduc2010use,wong2015clocom} conceptualize the tasks as information retrieval problems, which extract keywords from the source code and compose them into term-based summarization for a given code snippet.
% For instance, CloCom~\cite{wong2015clocom} employs code clone detection and natural language processing approaches to identify similar code segments and utilize comments from some segments to describe others effectively.
The second group of works~\cite{wang2021codet5,liu2022commitbart} applies neural machine translation techniques to code summarization domain.
The transformer architecture has been proven to be successful in many NLP tasks, thus, they are introduced to summarize source code snippets~\cite{guo2020graphcodebert,wang2021codet5,feng2020codebert}.
As an example, CodeT5~\cite{wang2021codet5} is pre-trained on the T5 model that has been proven to be powerful in solving machine translation challenges, and CodeT5 leverages the semantics-enriched code features, e.g., identifiers.
In addition to source code summarization, CodeT5 was further fine-tuned on the binary code dataset and the resulting framework is called BinT5~\cite{al2023extending}.
CodeBERT~\cite{feng2020codebert} is a bimodal pre-trained model for programming language and natural language and its applied to the automated code summarization task.
Different from the first two approaches that treat program code as natural language sequences, the third category of works~\cite{guo2020graphcodebert,chakraborty2022natgen,son2022boosting} distill program-specific features, e.g., control flow and data dependency, into code representations.
GraphCodeBERT~\cite{guo2020graphcodebert} incorporates the semantic structure of code by focusing on data flow relationships between variables rather than syntactic-level structures like abstract syntax trees (AST).


% \paragraph{Soft Prompt and Hard Prompt}

\paragraph{Prompt-based Learning}
% In a traditional supervised learning system for natural language processing, the dataset containing the input and output sample pairs are required to training and fine-tuning the system.
In a conventional supervised learning system designed for natural language processing, it is imperative to have a dataset comprising input and output sample pairs for the training and fine-tuning of the system~\cite{houlsby2019parameter}.
% The main issue with supervised learning is that to train a model it is necessary to have annotated data for the task, which for many tasks cannot be found in large amounts. 
The primary challenge associated with supervised learning is the requirement for annotated data to train a model. 
For numerous tasks, acquiring a substantial volume of annotated data proves to be a formidable obstacle.
% To address this issue, prompt-based learning methods for NLP attempt to circumvent this issue by instead learning a language model that learns only from sample input. 
% To tackle this challenge, prompt-based learning methods in NLP endeavor to bypass the need for extensive annotated data by training a language model that derives knowledge solely from sample inputs~\cite{min2021recent}.
% Among learning methods, manual prompt engineering, the most natural way to create prompts, is to manually create intuitive templates based
% on human introspection.
% Because the purpose of prompt construction is to find a method that
% allows an LM to effectively perform a task, rather than being for human consumption, it is not necessary to limit the prompt to human-interpretable natural language.
% Therefore, there are also methods that examine soft prompting that perform prompting directly in the embedding space of the model.
To address this challenge, prompt-based learning methods in NLP seek to eliminate the requirement for extensive annotated data by training a language model that acquires knowledge exclusively from sample inputs~\cite{min2021recent}.
Among these learning methods, manual prompt engineering is the most straightforward approach~\cite{liu2023pre}. 
It involves the manual creation of intuitive templates based on human introspection. 
Meanwhile, prompt construction doesn't necessarily need to adhere to human-interpretable natural language, as the primary goal is to enable the language model to effectively perform a task, rather than catering to human understanding. 
Consequently, there are also techniques that explore soft prompting~\cite{lester2021power}, wherein prompting is performed directly within the embedding space of the model.
% Automated prmptTemplate Learning
% cite: Multitask prompted training enables zero-shot task generalization
% Its versatility has led to widespread adoption in various NLP tasks. 
% cite: nlp tasks

% However, to employ prompting effectively with LLMs, it is necessary to carefully construct prompts, either manually or automatically, as these models do not interpret prompts in the same way as humans~\cite{reynolds2021prompt}. 
Nonetheless, for effectively prompting LLMs, it is crucial to meticulously devise prompts, through either manual or automated methods, as LLMs do not interpret prompts in the same way as humans~\cite{reynolds2021prompt}.
% cite: Prompt programming for large language models: Beyond the few-shot paradigm
% cite another: Making pre-trained language models better few-shot learners
While numerous successful techniques for prompt tuning exist, which optimize prompts in a continuous space using gradient-based methods~\cite{lester2021power}, this approach becomes less viable at larger scales due to the computational burden associated with calculating gradients~\cite{zhou2022large}. 
Although there are numerous automated prompt tuning approaches that involve optimizing prompts within a continuous space through gradient-based methods~\cite{lester2021power}, these approaches become increasingly impractical at larger scales due to the substantial computational overhead associated with gradient calculations~\cite{zhou2022large}.
% cite: https://arxiv.org/abs/2104.08691
% cite: https://arxiv.org/pdf/2211.01910.pdf
% Furthermore, increasing reliance on model access through APIs that lack gradient support further diminishes the feasibility of gradient-based optimization~\cite{peng2023instruction}. 
Moreover, the growing dependence on model access via APIs that lack gradient support further exacerbates the challenges associated with gradient-based optimization~\cite{peng2023instruction}.
% In this work, we focus on prompt search methods, encompassing prompt generation, prompt scoring, and prompt paraphrasing, to optimize instructions by directly exploring the hypothesis space of natural language.
In our study, our primary focus revolves around prompt search techniques, which encompass prompt synthesis, prompt scoring, and prompt paraphrasing based on LLMs and our binary summarization-specific evaluations. 
These methods are employed to enhance instructions by directly exploring the hypothesis space of natural language.
% cite: openAI api
% In this research paper, we integrate elements from discrete prompt search methods, encompassing prompt generation, prompt scoring, and prompt paraphrasing, in order to optimize instructions by directly exploring the hypothesis space of natural language. Unlike previous approaches that rely on specialized models for each component and heavily depend on human templates, we demonstrate that a single LLM can facilitate the entire search process.
% https://arxiv.org/pdf/2207.11680.pdf

% \subsection{Limitations of Existing Works}



==> sections/background_new.tex <==
\noindent\textbf{Large Language Models.} 
The widespread adoption of Large Language Models (LLMs) has been driven by significant advances in downstream tasks, e.g., machine translation and question answering~\cite{brown2020language}. 
% These advances have enabled the scaling of LLMs to encompass billions of parameters and the utilization of billions of training samples.
LLMs are initially trained to incorporate knowledge across domains, constrained by objectives like mask token prediction and next sentence generation~\cite{devlin2018bert}. 
Subsequently, LLMs are applied to downstream tasks through either fine-tuning or prompting strategies~\cite{liu2023pre}.
Fine-tuning involves the process of updating model parameters by minimizing the loss on task-specific datasets, but it is resource-intensive due to the necessity of weight updates and model training. 
% , ultimately optimizing performance on these downstream tasks. 
% However, it's worth noting that fine-tuning can be resource-intensive due to the necessity of weight updates and model training. 
% This can pose challenges when sufficient training data, hardware resources, or access to LLMs themselves are not readily available.
In contrast, the prompting approach involves directly executing model inference on LLMs without the need for retraining. 
% In order to provide LLMs with the context of downstream tasks, carefully crafted prompts are necessary to optimize LLMs' performance~\cite{liu2023pre}.
To equip LLMs with the necessary context for downstream tasks, the use of meticulously crafted prompts is imperative to optimize the performance of LLMs~\cite{liu2023pre,zhou2022large,pryzant2023automatic}.
% This practice is commonly referred to as in-context learning as we defined in~\S\ref{sec:definition}, as it equips LLMs with the necessary contextual information for task execution.

\paragraph{Automated Code Summarization}
% Research in automated code summarization concerns the study
% of systems and methods for expressing code fragments
% (in most cases methods or functions) written in a given
% programming language with a natural language expression that
% % encapsulates their functionality or purpose. 
Automated code summarization aims at articulating code fragments, typically methods or functions,  using natural language summaries that encapsulate their functionality or intended purpose~\cite{shi2022evaluation}.
% Recently, most of the works focus on source code summarization, inspired by natural language processing (NLP) approaches designed for text summarization, which in the last years are almost all based on neural
% architectures, and especially on transformer models
Recently, the predominant focus of this research has been on summarizing source code, inspired by natural language processing (NLP) techniques developed for text summarization~\cite{sharma2021survey}. 
The transformer architecture has been proven to be successful in many NLP tasks, thus, they are introduced to summarize source code snippets~\cite{guo2020graphcodebert,wang2021codet5,feng2020codebert}.
As an example, CodeT5~\cite{wang2021codet5} is pre-trained on the T5 model that has been proven to be powerful in solving machine translation challenges, and CodeT5 leverages the semantics-enriched code features, e.g., identifiers.
In addition to summarizing the source code, research attention has also been paid to summarizing binary code.
To the best of our knowledge, BinT5 is the only work in this direction, which finetunes CodeT5 on decompiled code~\cite{al2023extending}, and we have included BinT5 in our evaluations.
As mentioned in \S\ref{sec:intro} (\textbf{O$_1$}), all source and binary code summarization works use code comments created by developers as ground truth.
% Notably, in recent years, a substantial portion of these efforts has leaned heavily on neural architectures, with a particular emphasis on transformer models~\cite{guo2020graphcodebert,wang2021codet5,feng2020codebert}.
% Code summarization is the process of automatically generating concise and human-readable summaries or descriptions of code written in programming languages. 
% These summaries are intended to provide a high-level understanding of what a particular piece of code does, its functionality, and its purpose, without the need to read the entire codebase. 
% In the field of software engineering, this topic is of paramount interest due to its direct connection with the challenge of automating the generation of comments and documentation.
% Numerous endeavors have been undertaken in this area. 
% The majority of these studies~\cite{feng2020codebert,wang2021codet5,guo2020graphcodebert,ahmad2021unified,wang2022bridging} focus on generating summaries for small code blocks, such as individual methods. 
% This category also encompasses research on summarizing small code fragments~\cite{nazar2016source}, implementing code folding within integrated development environments~\cite{viuginov2019machine}, generating commit messages~\cite{liu2018neural,dong2022fira,liu2022commitbart}, and creating titles for online posts derived from code~\cite{du2019leopard}.
% To accomplish code summarization tasks, previous research endeavors have introduced three principal paradigms for modeling code semantics.
% As the first category, early works~\cite{haiduc2010use,wong2015clocom} conceptualize the tasks as information retrieval problems, which extract keywords from the source code and compose them into term-based summarization for a given code snippet.
% For instance, CloCom~\cite{wong2015clocom} employs code clone detection and natural language processing approaches to identify similar code segments and utilize comments from some segments to describe others effectively.
% The second group of works~\cite{wang2021codet5,liu2022commitbart} applies neural machine translation techniques to code summarization domain.
% The transformer architecture has been proven to be successful in many NLP tasks, thus, they are introduced to summarize source code snippets~\cite{guo2020graphcodebert,wang2021codet5,feng2020codebert}.
% As an example, CodeT5~\cite{wang2021codet5} is pre-trained on the T5 model that has been proven to be powerful in solving machine translation challenges, and CodeT5 leverages the semantics-enriched code features, e.g., identifiers.
% In addition to source code summarization, CodeT5 was further fine-tuned on the binary code dataset and the resulting framework is called BinT5~\cite{al2023extending}.
% CodeBERT~\cite{feng2020codebert} is a bimodal pre-trained model for programming language and natural language and its applied to the automated code summarization task.
% Different from the first two approaches that treat program code as natural language sequences, the third category of works~\cite{guo2020graphcodebert,chakraborty2022natgen,son2022boosting} distill program-specific features, e.g., control flow and data dependency, into code representations.
% GraphCodeBERT~\cite{guo2020graphcodebert} incorporates the semantic structure of code by focusing on data flow relationships between variables rather than syntactic-level structures like abstract syntax trees (AST).


==> sections/case-study.tex <==
% \paragraph{A Close Look at LLM-generated Summaries}
% To what extent can LLMs understand binaries?
% \Xin{This paragraph can be an individual case study section.}
\Xin{Move to evaluation section.}
After obtaining the statistical results, there are two more questions to be answered: (\textit{i}) To what extent, can LLMs understand binary code (specifically decompiled code) and (\textit{ii}) how to understand the reported scores?
To answer these questions, we perform case studies on the LLM-generated summaries and their calculated scores.
In particular, we focus on the samples that LLMs achieved the best, median, and lowest scores, which fall into 100-th, 50-th, and 0-th text similarity score percentile among all the binary code samples.
We argue that we can gain distribution insights across extreme and median cases via such an investigation, as well as understand LLMs' robustness on binary code comprehension.
% \autoref{} presents the examples with ground truth summaries, LLM-generated summaries, and evaluation scores.
% examples in the appendix about the individual examples

% Based on this investigation, we first examine how LLMs perform when given binary code input in different representations.
\paragraph{Important of Source-level Symbols and Information}
\autoref{tab:source-code-example} presents the summaries generated for the source code samples.
Overall, we observe that LLMs can capture most of the semantics in the source code.
For samples with the best and median scores, there is notable semantic overlap between LLM-generated and ground-truth summaries.
For example, the generated summary for function 1 covers the key semantics of ``hash table'', ``free the memory'', and ``if hash table exists'', which also show in the ground-truth summary.
Even for the sample with the worst score, we still observe that LLMs capture partial semantic information in the input code.
In addition, we observe similar good performance from the decompiled code with the debugging symbols in \autoref{tab:decomp-debug-example}, in which LLMs can capture the semantics of samples that achieve the best and median scores, while LLMs can fail to understand decompiled code semantics for these with the lowest scores, such as function 4 in \autoref{tab:decomp-debug-example}.
However, for decompiled code from stripped binaries, LLMs cannot generate summaries explicitly matching the ground-truth summaries, as shown in \autoref{tab:decomp-stripped-example}.
For example, the generated summary for function 2 in \autoref{tab:decomp-stripped-example} can capture the overall semantic operation of file name canonicalization, but it misses many details of this operation, such as removing dots and repeated file name separators as demonstrated in the ground-truth summary.
For function 3, the generated summary can only include the ELF file format and lose all semantic information.
Such a semantic gap between ground-truth and LLM-generated summaries in \autoref{tab:decomp-stripped-example} comes from the loss of high-level semantics preserved in the symbol names, e.g., functions and variables names.

\finding{The loss of source-level symbol and information leads to degradation of LLM-generated summaries for decompiled code, which fail to cover sufficient semantics of binary code.}

\paragraph{Operational Description of Low-level Binary Code Representations}
For low-level code, including IR code, assembly code and raw bytes, we find LLMs mostly focus on describing the operations performed by the input code without high-level summaries with semantic emphasis.
For example, \autoref{tab:ir-code-example} presents the summaries and evaluation scores of the IR code.
The generated summaries in different text similarity scores mostly describe the operations of data movement, arithmetic calculations (e.g., addition and subtraction), memory loading/writing, and data flow transformation (e.g., jump operation).
Similarly, we also observe such descriptions for assembly code and raw bytes as shown in \autoref{tab:assembly-example} and \autoref{tab:raw-bytes-example}.
However, the ground-truth summaries for these binary code are most about their high-level functionalities.
Compared to the human-readable decompiled code that resembles the structure of pseudo-source code, the low-level code loses the code structure information and focus on low-level program behavior, which results in the semantic gap between ground-truth and LLM-generated summaries.
In addition to the semantic gap, we also find that the assembly code tends to be much shorter than IR code and raw bytes, and LLMs can capture some high-level data structure in assembly code, such as strings in function 1 of \autoref{tab:assembly-example}.

\finding{For low-level binary code representations, e.g., assemble and IR code, LLMs generate summaries that mostly describe the low-level operations, such as data movement and arithmetic calculations, that cannot represent the high-level code functionalities.}

\paragraph{Implicit Code Lifting of Raw Bytes}
While investigating the LLM-generated summaries of raw bytes, we observe that they carry the higher level summaries of code semantics, instead of simply describing the raw bytes.
We argue that there exists some implicit code lifting and reason process when LLMs summarize the binary raw bytes.
For example, in function 2 of \autoref{tab:raw-bytes-example}, the summary describes the operations of the stack frame, function calls, loops with conditional jumps, and arithmetic operations.
However, when providing raw bytes as the input to LLMs, we directly ask LLMs to generate code summaries without requesting code lifting (e.g., converting raw bytes into the higher level assembly code or IR code).
Surprisingly, instead of describing the byte-level information, LLMs seem to have lifted the raw bytes into high-level representations which can represent the above-mentioned operations.
For function 1 in \autoref{tab:raw-bytes-example}, the generated summary even includes the semantics of high-level data structure, i.e., strings, and file path properties.

\finding{For raw bytes, LLM-generated summaries exhibit the implicit process of lifting the bytes to higher level code, and the summaries even include the semantics of the string data structures and file path properties.}

\paragraph{Necessity for Semantically Evaluating Summaries}
As discussed in \S\ref{sec:challenge} and \S\ref{sec:solutions}, the binary code summaries are in natural languages that present semantics in a fuzzy manner.
The widely used summarization evaluation metrics, including BLEU, METEOR, and ROUGE-L, calculate similarity scores based on exactly matched n-grams in ground-truth and generated summaries as presented in \S\ref{sec:exact-matching-metrics}.
However, we observe that they cannot accurately measure the quality of generated summaries. 
For example, for function 2 in \autoref{tab:source-code-example}, BLEU, METEOR, and ROUGE-L are all calculated as 0 without syntactical overlaps between ground-truth and LLM-generated summaries .
Nevertheless, these summaries present close semantics, such as ``routine'' and ``function'' as well as ``a filename'' and ``the name of the file''.
These words/phrases are syntactically different, but semantically the same, which are widespread in the code summaries.
Different from the n-gram-matching best metrics, our semantic evaluation metric (\S\ref{sec:testing-eval}) computes semantic similarity by first generating semantic embeddings of summaries and then calculating their embedding distance at the semantic level.
Therefore, we argue that our semantic evaluation metric is more suitable for evaluation binary code summaries than the n-gram matching metrics.

\finding{Our semantic evaluation metric can capture the essential semantics of binary code summaries and calculate similarity at semantic level, which is more suitable for our binary code summarization task than the n-gram-matching metrics, e.g., BLEU, METEOR, and ROUGE-L.}

% \paragraph{Malicious Binary Code Rewriting}
% Manipulating Decompiled Code to Fool LLMs

% \paragraph{LLM Finetuning}
% \paragraph{Source-Binary Code Semantic Gap}
% Simply fine-tuning small LLMs won't help binary code understanding

==> sections/dataset.tex <==

\subsection{Limitation of Existing Dataset}

\bintf is a binary code summarization tool finetuned from CodeT5-base model. 
It has the following issues. 
First, it only focused on Ghidra-generated decompiled code which doesn't give general perfomance for general decompiler-output code.
However, we observed that the code generated from different compilers is dramatically different. 
For example, \xy presents the code generated by Ghidra and Hex-rays.
Second, the dataset only covers x86-32 binaries, which are extracted from BinSwarm~\cite{ahmed2021learning}.
Third, \bintf compares the summarization performance across optimization levels but its dataset is imbalanced regarding optimization levels, i.e., it's binaries with different optimization levels following abnormally distribution.
For example, the decompiled functions of -O0, -O1, -O2, and -O3 optimization levels follow the rough ratio of 1:2:6:2.
However, compiling source projects into binaries with different optimization levels usually render far more -O0 functions compared to -O1~-O3~\cite{jin2022symlm}.
Therefore, we believe training on such an imbalanced dataset doesn't give us the fair performance comparison across different optimization levels.

Besides \bintf, there are also works for binary code semantic modeling which maps semantic encodings into function names~\cite{he2018debin}
For example, SymLM models binary code semantics preserved in calling context and execution behaviors with a pretrained large language model.
However, the function names generated by such works give very concentrated and short semantic descriptions but fail to provide enough details.

\subsection{Binary Compilation and Stripping}

\input{tables/src-projects}

To obtain the dataset with general representations, we opt to compile the open-source projects into various binaries with different compilation settings.
Specifically, we collect 44 open-source projects from GNU Software~\cite{GNUSoftware}, including these that are widely used in binary reverse engineering research~\cite{jin2022symlm}, such as coreutils, binutils, and findutils.
\autoref{tab:source-projects} list all the projects used in our dataset.
We compile the projects into 4 computer architectures (x86, x64, ARM, and MIPS) and 4 optimization levels (O0-O3), which results in 8,760 unique binaries.
We also apply obfuscation techniques to further obfuscate the binary code.
Specifically, we obfuscate binaries with the LLVM Obfuscator and enable the \xy options.

Our evaluation environment is a 64-bit Ubuntu desktop. 
Compiling and stripping binaries with different computer architectures as the host machine require cross compilers and cross-stripping tools.
For this, we build a cross-compilation and cross-stripping tool.
To compile the binary on a 64-bit Linux machine, we use cross-compilers, \texttt{arm-linux-gnueabihf-gcc} and \texttt{mipsel-linux-gnu-gcc} for ARM and MIPS binaries.
For binary stripping, we remove all symbol names using the \texttt{strip} command, in which we used \texttt{arm-linux-gnueabihf-strip} and \texttt{mipsel-linux-gnu-strip} to strip the ARM and MIPS binaries.

\subsection{Ground Truth Comment Extraction and Preprocessing}
To collect the ground-truth comments, we parse the source files in each project.
% For this, we have two design choices
For this, we search for open source tools for source code parsing and find three potential candidates, that is, \texttt{comment\_parser}, \texttt{srcML}, and \texttt{pycparser}.
\texttt{srcML} requires converting source files into XML files, which needs additional parsing efforts.
\texttt{pycparser} requires preprocessing source files, which requires library files.
Therefore, we leverage \texttt{comment\_parser}, which is the lightest among the tools.

\texttt{comment\_parser} extracts comments from source files with corresponding line numbers.
However, it cannot automatically identify the function associated with each comment.
To address this issue, we design the \xy algorithm to associate comments with each function.
Although one function comment convention~\cite{doc-functions-c-cpp} is to put function descriptions in header files, our investigation of 450 randomly selected source functions across different source projects shows that (1) most functions are not commented on, (2) developers rarely comment on function declarations in header files, and (3) even when developers comment on function declarations in header files, they usually reuse such comments and or add more information to comment function implementations in source files.
Therefore, we focus on parsing comments in the source files.

We first extract comments and their line numbers from the source files using the \texttt{comment\_parser}.
We then iterate each comment within the source files.
We check whether there is a function signature below each comment, which is treated as the function descriptions for identified functions.
However, some functions defined in the source files may not be included in the binaries, and there may be some parsing errors.
To address such issues, we cross-validate the functions from the debugging symbols.
That is, we keep descriptions only for functions that appear in the binaries.

During source file parsing, we also find that some functions, such as the main functions, are defined multiple times in the same source file or across multiple source files.
To align the functions in the source code and those in the binaries, we match source function names and functions in the binaries with debugging symbols.
Therefore, it is challenging to identify the correct matching if the functions with the same name are given different comments.
% If the definitions of the same functions are with different comments, it's hard to determine which description correspond to the functions in binary.
We define such comments as ambiguous comments, and the functions with ambiguous comments are removed from our dataset.
For example, in the \texttt{poke-2.4} project, our source code parser identifies 1,026 unique functions with comments.
144 functions are defined multiple times, and 30 functions are defined with different comments, i.e., with ambiguous comments.
We duplicate the functions with the same function comments and remove the functions with ambiguous comments.
This process results in the function comment dataset.
For example, the number of unique functions after cleaning is 996.
% 246 functions are defined in multiple times, e.g., defined across multiple source files.
% 103 functions are with ambiguous comments.
Overall, our source project parser extracted 40,046 unique functions with comments from source projects and 780 functions are with ambiguous comments.
After cleaning, there are 39,266 functions in the dataset.
% We remove ambiguous descriptions 

Although functions are defined in source projects, they may not be used in compilation.
For example, developers can use the \texttt{\#if} macro to selectively compile functions into binaries.
To remove such uncompiled functions, we first collect all functions from binaries compiled from each source project.
% This results in 161,615 functions.
We use Ghidra to analyze the DWarf entries of binaries and identify functions and their names, which results in 161,615 functions.
For binaries from a specific project, we identify all unique functions by name and then check the overlap between binary functions and source functions based on function names.
\Xin{TODO: draw a figure to show such process}.
For example, for the 996 unique source functions with comments defined in the \texttt{poke-2.4} project, 530 functions are compiled into binaries.
This matching process identified 18,239 source functions compiled into binaries.

\subsection{Data Extraction}

After identifying the comments for functions, we extract the raw bytes, assembly code, IR code, and decompiled code from the ELF files in xy steps.
% First, we identify function start and end adresses for the functions with comments by parsing the DWARF entries.
% Second, we extract the raw bytes of functions from the \texttt{.text} section based on function addresses.
% For disassembly code, we leverage the 

\paragraph{Decompilation}
With the diverse binaries compiled from various compilation settings, we decompile binaries with Ghidra and Hex-Rays, which are the most popular decompilers among reverse engineers and academic researchers. % NFRE uses Hex-rays to obtain the assembly code. 
For example, NFRE~\cite{} models the function semantics for stripped binary function with the assembly code generated by IDA.
varBERT~\cite{} predicts variable names by learning local variable semantics with Ghidra output.
Therefore, we investigate whether LLMs can understand binary code semantics by decompiling binaries with these two decompilers.
For Ghidra and Hex-Rays, we use their Python APIs \texttt{ghidra.app.decompiler.DecompInterface} and \texttt{idaapi.decompile} to iteratively decompile functions in the \texttt{.text} segment, respectively.
% For Hex-Rays, we the IDA Python API \texttt{idaapi.decompile} to decompile 


\paragraph{Disassembling and Raw Byte Extraction}
To extract the assembly code representations of binary functions, we first identify start and end addresses of the functions by parsing the DWARF entries to get the \texttt{DW\_AT\_low\_pc} and \texttt{DW\_AT\_high\_pc} attributes.
With the addresses, we disassemble binary functions with \texttt{capstone.Cs.disasm\_lite} API.
The function addresses are also used for raw bytes extraction from binaries, where we directly read the bytes based on addresses.

% \paragraph{}

\paragraph{IR Code Extraction}
For IR code extraction, we use IDA IR, i.e., IDA microcode

\subsection{Code Comment Classification}

Developers generates descriptive comments for a segment of source code in human languages. It is worth noting that code comments serve various purposes in practice.
For instance, some comments elucidate the functioning of functions or source files, whereas others provide the action items for code improvement, e.g., bug fix notes.
Previous works have found that incorporating code comments withAre we building on the rock? on the importance of data preprocessing for code summarization poor quality into the code summarization dataset can either hurt the summarization capacities or not reveal the true performance of the well-developed tools~\cite{chen2021my}.



==> sections/eval-RQ1-old.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/cross_representation_violin.pdf}
  \caption{LLM Performance across Code Representations. For decompiled code, ``decompiled'' and ``stripped'' refer to these with and without debugging symbols.
  % We compare LLMs' performance on source code, decompiled code from binary with debugging symbols (Debug), decompiled code from stripped binaries (Stripped), IR code, assembly code, and raw bytes.
  }
  \label{fig:cross-representation}
\end{figure}



% figure: different code representations for the models

% To understand how LLMs can understand binary code, we compare their performance in the different representations of binary code along with the source code and present the results in \autoref{fig:cross-representation}.
To answer \textbf{RQ1}, we first evaluate the performance of LLMs on different representations of binary codes, including decompiled code, IR code, assembly code, and raw bytes along with source code, and present the results in \autoref{fig:cross-representation}.
% Here, we exclude BinT5's performance as it only accepts decompiled code.
Among the different code representations, we found that LLMs perform the best in source code, achieving an average semantic similarity score of 0.474.
% It outperforms the decompiled code from binaries with debugging symbols, which has the average text similarity of 0.449.
% For decompiled code, we have observed a significant performance degradation when symbols are stripped from binaries, i.e., reducing the semantic similarity score from 0.449 to 0.202.
For decompiled code, we observe a significant performance degradation when symbols are stripped from binaries, reducing the semantic similarity score from 0.449 to 0.202 (55.0\% decrease).
\result{Stripping debugging symbols significantly loses decompiled code semantics by 55.0\%.}
% the information loss during the compilation and decompilation process, though all the symbol names and type information are preserved in the decompiled code.
% However, this decompiled code significantly outperforms its variant from stripped binaries that achieves 0.202 average text similarity, which meaning removing the debugging symbols results in a 55.0\% information loss.
% Even with such a huge information loss, we still find that the decompiled code without symbols still outclasses the other binary code representations.
% Specifically, LLMs achieve 0.188, 0.185, and 0.188 average text similarity scores on assembly code, IR code, and raw bytes.
Even with such a significant information loss, decompiled code without symbols still outperforms the other binary code representations. 
LLMs achieve average text similarity scores of 0.188, 0.185, and 0.188 on assembly code, IR code, and raw bytes, respectively.
% In addition to text similarity, we have the similar observations on the other evaluation metrics.
% Similar observations were made regarding the other evaluation metrics as well.
% For example, the average METEOR scores are 0.167, 0.141, 0.102, 0.052, 0.0663, and 0.063 for source code, decompiled code (debugging), decompiled code (stripped), IR code, assembly code, and raw bytes, respectively.
Comparable trends are identified in other evaluation metrics, e.g., the mean METEOR scores are 0.167, 0.141, 0.102, 0.052, 0.066, and 0.063 for source code, decompiled code (debug), decompiled code (stripped), IR code, assembly code, and raw bytes, respectively. \looseness=-1
% With this observation, we focus on presenting 
% Therefore, we argue that the decompiled code can serve as the best option, compared to the other binary code representations, for LLMs to understand when given the stripped binaries.

\result{LLMs perform the best on decompiled code compared to IR code, assembly code, and raw bytes.}



\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/cross-model.pdf}
  \caption{Performance across Different LLMs. The decompiled code from binaries with debugging symbols (debug) and stripped binaries (stripped) are compared.
  % \Xin{Reduce outliers to accelerate rendering}}
  }
  \label{fig:cross-model}
\end{figure}

% figure: different LLMs for decompilations

This observation also motivates us to conduct an in-depth study of the decompiled code comprehension capacity of different LLMs. \autoref{fig:cross-model} presents the performance of different LLMs on understanding the decompiled code from binaries with debugging symbols and stripped binaries.
We then set up to understand which LLM performs the best on decompiled code with debugging symbols and decompiled code from stripped binaries.
On one hand, for the decompiled code with debugging symbols, we observe the ChatGPT model performs the best achieving 0.543 average text similarity score, while BinT5 performs the worst with 0.115 similarity score on average.
Compared to Llama 2 models, Code Llama models achieve 4.57\%, and 11.3\% better performance on the 7B and 13B models, respectively, which indicates Code Llama's fine-tuning on code corpora helps it comprehend decompiled code.
On the other hand, for the decompiled code from the stripped binaries, we find that the Code Llama models outperform all other LLMs achieving 0.284 and 0.283 average text similarity scores for 7B and 13B models, while the BinT5 model still gets the worst text similarity score of 0.114.
% However, we find the performance gap between 
Moreover, Code Llama models outclass Llama 2 model by 12.3\% and 22.0\% on the 7B and 13B models.
For BinT5, we find it achieves the almost same performance on decompiled code with and without debugging symbols while other LLMs achieve very different performance.
Moreover, we observe BinT5 cannot properly understand decompiled code semantics (see \S\ref{} for more details) though it's fine-tuned from the CodeT5 model with decompiled code samples.
Therefore, without further notice, we exclude BinT5's summaries from our further studies.
Moreover, we find it's summaries contain some outliers with over 0.8 text similarity scores and out investigation shows that they are potentially leaked in BinT5's training set (See \S\ref{sec:bint5-outlier} for more discussions).
\result{ChatGPT and Code Llama models achieve the best text similarity scores of 0.543 and 0.283 for understanding decompiled code with debugging symbols and that from stripped binaries, respectively.}
\result{Code Llama models, fine-tuned from  Llama 2, consistently outperform Llama 2 on decompiled code achieving up to 22.0\% better performance. However, simply finetuning CodeT5 cannot result in a good performance of BinT5.}

% figure: different ground truth summary length v.s. similarity scores

% To further study to what extent the 


==> sections/eval-RQ2-old.tex <==
\subsection{RQ2: Diverse Binaries}
\label{sec:eval-RQ2}
\input{sections/eval-RQ2}
% figure: cross architecture, which computer architecture of binaries is the best

\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/cross-arch.pdf}
  \caption{Performance across Computer Architectures}
  \label{fig:cross-arch}
\end{figure}


% figure: cross optimization levels



To understand how the diverse binaries compiled from various compilation settings can affect LLM's comprehension, 
we examinate LLMs' performance of binaries compiled into different computer architectures and optimization levels.
We exclude the calculated scores of BinT5 as we find that it cannot properly understand the decompiled code semantics, which has been discussed in \S\ref{sec:eval-RQ1}.

% we first study their performance on binaries with different computer architecture.
\autoref{fig:cross-arch} presents the performance on decompiled code across different architectures, i.e., x86, x64, ARM, and MIPS.
For the decompiled code with debugging symbols, the average text similarity scores for decompiled code from x86, x64, ARM, and MIPS binaries are 0.483, 0.503,  0.497, and 0.485, respectively.
The performance on x64 binaries outclasses these on x86 binaries by 4.14\%.
For the decompiled code from stripped binaries, the similarity scores are 0.262, 0.299, 0.276, and 0.304 for the x86, x64, ARM, and MIPS binaries, respectively.
Different from the marginal outperformance in decompiled code with debugging symbols, decompiled code from stripped MIPS binaries obtains 16.0\% better text similarity scores compared to x86 binaries.
% Thus, we observe that LLM's performance on 
\result{When given decompiled code with debugging symbols, LLMs performs the best on x64 binaries (up to 4.14\% outperformance). For decompiled code from stripped binaries, MIPS is the best for LLMs to understand (16.0\% better than x86 binaries). In both cases, LLMs perform the worst on x86 binaries.}

\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/cross-opt.pdf}
  \caption{Performance across Optimization Levels}
  \label{fig:cross-opt}
\end{figure}

\autoref{fig:cross-opt} presents LLMs' performance on decompiled code from binaries with four optimization levels.
For the decompiled code with debugging symbols, our target LLMs achieve 
0.481, 0.477, 0.477, and 0.474 average text similarity scores for O0, O1, O2, and O3 binaries.
For the decompiled code from stripped binaries, the text similarity scores of these binaries are 0.269, 0.268, 0.266, and 0.270 on average.
For both types of decompiled code, we observe the marginal performance difference cross optimization levels, e.g., performance between O0 and O3 binaries is 1.47\%.
\result{LLMs show marginal performance gap cross different optimization levels, e.g., 1.47\% different text similarity scores between O0 and O3 binaries.}

==> sections/eval-RQ3-old.tex <==

% fig: Cross Decompilers
\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/cross-decompiler.pdf}
  \caption{Performance across Different Decompilers}
  \label{fig:cross-decompiler}
\end{figure}

While we have identified the decompiled code to be the best binary code representation for LLM to understand, we further investigate which decompiler generates the optimal output for code comprehension.
\autoref{fig:cross-decompiler} presents the LLMs' performance of the output decompiled code from three different decompilers, i.e., Ghidra, Hex-rays (IDA), and Angr.
Among the three decompilers, we observe that Hex-rays consistently outperforms the other two decompilers in decompiled code both with debugging symbols and from stripped binaries.
Specifically, LLMs achieve 0.444, 0.468, and 0.384 average text similarity scores on binaries with debugging symbols for Ghidra, Hex-rays, and Angr, respectively, in which Hex-rays outperforms Ghidra by 5.41\% and Angr by 21.9\%.
For decompiled code from stripped binaries, the average text similarity scores for these three decompilers are 0.173, 0.278, and 0.232, where Hex-rays achieves the more significant outperformance, e.g., 60.7\% and 19.8\% better than Ghidra and Angr outputs respectively.
We believe the outperformance of Hex-rays comes from the higher quality of generated decompiled code, which is reasonable considering Hex-rays is a commercial decompiler.
% it's reasonable to observe such consistently better
Moreover, different from the decompiled code with debugging symbols, Angr outperforms Ghidra on understanding stripped binary decompiled code, achieving 34.1\% better text similarity scores.
However, we observe that Angr is significantly slower than Ghidra and Hex-rays.
% Based on observation our dataset generation process,
For example, Angr requires about 15$\times$ more decompilation time than Ghira with setting the \texttt{CFGFast} analysis for Angr, while Ghidra and Hex-rays consume the comparable decompilation time. 

\result{Compared to Ghidra and Angr, Hex-rays generated decompiled code consistently obtain the betterscores for LLM summaries with up to  60.7\% better text similarity score. 
% Ghira and Angr achieve the second best scores on decompiled code with debugging symbols and from stripped binaries respectively 
}

\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/cross_stripping.pdf}
  \caption{Performance on Decompiled Code with Symbols Stripped. We exclusively replace function names (w/o Func Name), variable names (w/o Var Name), and data types (w/o Type) with meaningless symbols in the decompiled code which original has all symbols (Original). We compare their performance with decompiled code from stripped binaries whose symbols are all stripped (w/o All)}
  \label{fig:cross-stripping}
\end{figure}

In \S\ref{sec:eval-RQ1}, our evaluations show that losing the debugging symbols can significantly degrade LLMs' performance in understanding decompiled code.
Meanwhile, the binary reverse engineering community has put numerous efforts in recovering symbols from stripped binaries to enhance binary code semantics~\cite{banerjee2021variable,jin2022symlm,pei2021stateformer}.
For example, StateFormer~\cite{pei2021stateformer}, VarBERT~\cite{banerjee2021variable}, and SymLM~\cite{jin2022symlm} recover data types, variable names,  and function names from stripped binaries using binary-specific LLMs.
Based on this observation, we investigate what information, including data types, variable names, and function names, in decompiled code contributes the most to binary code semantics.
For this, we strip the information by exclusively replacing each of these three sets of information from decompiled code with debugging symbols by meaningless symbols.
For function names, we replace the original names with symbol \texttt{Fun\_addr} in which \texttt{addr} is the address of functions.
For variable names, we replace the original names with symbol \texttt{Var\_idx} where \texttt{idx} is the index of variables in the function.
For data types, we replace the original types with symbol \texttt{undefined}.
With this replacing process, we generate three decompiled code datasets, in which we only change the corresponding information in the decompiled code.

\autoref{fig:cross-stripping} presents LLMs' performance on the different decompiled code dataset we have created by replacing symbols with meaningless ones.
Compared to the original decompiled code with all symbols, the performance degradations of exclusively removing meaningful function names, variable names, and data types are 30.3\%, 30.0\%, 19.5\%, respectively, while removing all symbol names results in a degradation of 43. 7\%.
Since removing function names reduces LLM's performance the most, we argue that function names contribute more to the decompiled code semantics compared to variable names and data types.
Meanwhile, variable names contribute to the decompiled code semantics to the close extend to function names, while data types are less significant for binary code understanding.
Considering function and variable names convey semantics explicitly while data types contains implicit semantic information, we argue that LLMs are good at capturing explicit semantic information in binary code.
% the semantically rich nature of function and variable names 
% Meanwhile, replacing data types leads to the smallest degradation, meaning the data types can 
% 0.498 -> original, func name -> 0.34709, var name -> 0.34723, type -> 0.4011, all -> 0.28014

% fig: What Symbols Contribute Most to Binary Semantics? 
\result{Function name contributes to decompiled code semantics the most, e.g., reducing LLM's performance by 30.3\%, while data types are least significant for binary code understanding with LLMs.}

% example of foul LLMs

==> sections/eval-RQ4-old.tex <==
% figure: prompt engineering effects

\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/cross_prompting.pdf}
  \caption{Performance on Different Prompt Engineering Techniques}
  \label{fig:cross-prompting}
\end{figure}

In our evaluation, we focus on probing LLM's zero-shot learning capacities of binary code understanding with our proposed prompt synthesis and optimization approach (\S\ref{sec:prompt-engineering}).
We also examine whether the other prompt engineering techniques can help LLMs understand binary code.
Specifically, we focus on two popular techniques, including few-shot learning and chain-of-thought prompting.
Few-shot learning for LLMs was initially introduced to enhance the generalizability of GPT-3 for tasks beyond its primary domain~\cite{brown2020language}. 
This is achieved by imparting the model with contextual knowledge through in-context instructions, which is commonly referred to as zero-shot learning, or through demonstration samples, a technique known as few-shot learning.
% Specifically, in-context learning involves adding a piece of system instruction $\mathcal{I}$ along with zero or $n$ in-context demonstration pairs ($\mathcal{X}_{d}$, $\mathcal{Y}_{d}$), where $\mathcal{X}_{d}$ and $\mathcal{Y}_{d}$ are sample inputs and outputs, before the test input:
To be more specific, few-shot learning entails the inclusion of a system instruction $\mathcal{I}$ along with either $n$ in-context demonstration pairs ($\mathcal{X}_{d}$, $\mathcal{Y}_{d}$), where $\mathcal{X}_{d}$ and $\mathcal{Y}_{d}$ represent sample inputs and outputs. This augmentation occurs prior to the introduction of the test input:

\begin{equation}
    x = \{\mathcal{I}; (x_d^{i}, y_d^{i})^{n}; x_{t}\}
\end{equation}
\noindent where the system instruction and demonstration samples are concatenated with the test input $x_{t}$ to form the query input $x$.
\autoref{fig:few-shot} presents the example prompt that we used to perform few-shot learning with the GPT-4 model.
Instead of using fixed demonstration examples, we randomly sample two pairs of example binary functions and summaries for each test binary code to avoid LLMs learning the unchanged pattern in the demonstration examples.
Chain-of-thought prompt is proposed to resolve complex reasoning problems by breaking them down into intermediate steps~\cite{wei2022chain}.
In the context of binary code understanding, we ask LLMs to perform an additional step of reasoning the input code semantics before generating the final code summaries.
For this, we first send one request asking LLMs to reason about the code semantics, in which we use the popular reasoning prompt ``Let’s think step by step''.
Upon receiving the response, we parse the generated code reasoning results and concatenate them into the second request inquiring about the code summaries.
\autoref{fig:cot} presents the sample of our chat-of-thought prompts for GPT-4 model.
To test these advanced prompt engineering techniques, we use the decompiled code samples from stripped binaries due to several reasons.
First, compared to decompiled code with symbols, our test decompiled code is more challenging to comprehend, demanding a deep understanding of the essential code semantics.
Second, the test-decompiled code contains less high-level semantic information, e.g., function and variable names, which can potentially distract LLMs in reasoning code semantics.
Finally, real-world binaries are commonly in stripped binary format, for which code summaries are more helpful.
For zero-shot learning, as exemplified in ~\autoref{fig:zero-shot}, we directly concatenate the prompt with the test code to generate the request.

% \Xin{Motivate why we present decompiled code (stripped) performance. Stripped contains less semantics -> COT may help it reasoning as it's similar to math problems. -> Need to explain what COT is and how it can help solving reasoning-intensive tasks.}
% figure: model efficiency
\begin{figure}
  \centering
  \includegraphics[width=0.35\textwidth]{figures/prompting-token-distribution.pdf}
  \caption{Prompt Length Distribution of Different Prompt Engineering Techniques}
  \label{fig:token-num-distribution}
\end{figure}

\autoref{fig:cross-prompting} presents the performance of LLMs when using different prompt engineering techniques.
Among the prompting methods, we find that zero-shot, few-shot, and chain-of-thought prompts achieve 0.282, 0.312, and 0.271 text similarity scores on average, respectively.
Compared to zero-shot learning, demonstration examples in few-shot learning can improve the performance of LLMs by 10. 6\%.
Chain-of-thought reasoning does not improve models' performance.
While the few-shot learning method outclasses both zero-shot and chain-of-thought prompting, it has one notable drawback, e.g., the high prompt cost.
\autoref{fig:token-num-distribution} presents the prompt length distribution of zero-shot, few-shot, and chain-of-thought prompt engineering, in which few-shot prompts have much more input tokens.
Specifically, the median numbers of tokens for zero-shot, few-shot, and chain-of-thought prompts are 244, 1763, and 944.
The more input tokens, the higher the computational cost.
For example, the few-shot prompting on GPT-4 requires an extra 0.122 US dollars per prompt compared to zero-shot prompting on average.
Considering the scale of binary code summarization tasks, such as our evaluations, zero-shot learning can be a better solution based on the balance of performance and cost.

\result{Compared to zero-shot learning, few-shot learning can improve LLMs' performance on binary code summarization while it significantly increases the cost, e.g., requiring an extra 0.122 US dollar per prompt for GPT-4. Chain-of-thought does not improve LLMs' performance while increasing the cost as well.}

\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{figures/model-efficiency.pdf}
  \caption{Efficiency of Our Target Models. }
  \label{fig:efficiency}
\end{figure}

Different LLMs have different model sizes and parameters, which result in the different runtime overheads.
Thus, we evaluate the efficiency of our target models in terms of inference time cost.
% Instead of directly comparing our target models' 
To give a fair comparison, we first compare ChatGPT and GPT-4 inference time, and then we measure and compare the overhead of the rest LLMs, because we have used different evaluation environments for these two sets of LLMs (i.e., OpenAI APIs for ChatGPT/GPT-4 and a cloud server for the rest models).
\autoref{fig:efficiency} presents the distribution of inference time per binary code sample of OpenAI models and open-source LLMs.
For OpenAI models, the median inference time for ChatGPT and GPT-4 are 1.07 and 3.10 seconds per sample.
In terms of Llama Models, it takes 0.833, 1.123, 1.292, and 1.715 seconds for Llama 2-7B, Llama 2-13B, Code Llama-7B, and Code Llama-13B models to generate one summary.
Interestingly, we found the fine-tuned Code Llama models take more time for inference compared to Llama 2 models, and the inference time of Llama 2 models is more diverse compared to Code Llama models.
BinT5 is the fastest model among all our target LLMs, which takes 0.216 seconds per sample.
% For our target LLMs, we first compare GPT-4 and ChatGPT because we have used the OpenAI APIs to perform inference.
% Next, we compare 
In addition to the time cost, we also observe the memory consumption difference among the open source LLMs.
Specifically, the 7B and 13B Llama models occupy 42.6GB and 61.9GB of GPU VRAM, respectively, while the BinT5 model only takes 3.4GB of VRAM.
\result{Compared to GPT-4, ChatGPT is 2.9$\times$ faster in generating binary code summaries. For open source LLMs, the 7B Llama models are about 1.5$\times$ faster than the 13B models, while BinT5 is the fastest model among all the models. }

% Such a 

% 42631MiB for code-llama-7b
% 61969MiB for code-llama-13b

==> sections/introduction.tex <==


%Binary code analysis plays a crucial role in computer security. As more of our world runs on software, from critical systems to everyday apps, understanding the code that powers these systems is essential. Serving as the nexus between the intentions of human developers and the cold precision of machine language, binary code analysis facilitates our endeavors in both offensive and defensive security~\cite{shoshitaishvili2016sok}. In the domain of defensive security, thorough binary code analysis aids in identifying vulnerabilities~\cite{eschweiler2016discovre,luo2023vulhawk}, uncovering hidden backdoors~\cite{shoshitaishvili2015firmalice}, and ensuring that software behavior aligns with its intended design. Conversely, in offensive security, understanding binary code is crucial for exploiting vulnerabilities, developing sophisticated malware~\cite{mohan2012frankenstein}, and advancing penetration testing techniques~\cite{szekeres2013sok}. Yet, to be genuinely transformative in these realms, a deep, semantic understanding of binary code is vital---one that extends beyond mere pattern recognition and delves into the embedded logic, intent, and function.

Binary code analysis is pivotal in the realm of computer security, holding immense significance as the backbone of our increasingly software-dependent world. Whether it is the critical systems safeguarding our data or the ubiquitous apps that pepper our digital lives, delving into the underlying code is indispensable. This analytical process acts as a critical interface between human creativity and the rigid exactitude of machine language, serving as a linchpin in both offensive and defensive security efforts~\cite{shoshitaishvili2016sok}. In the domain of defensive security, thorough binary code analysis aids in identifying vulnerabilities~\cite{eschweiler2016discovre,luo2023vulhawk}, uncovering hidden backdoors~\cite{shoshitaishvili2015firmalice}, and ensuring that software behavior aligns with its intended design. Conversely, in offensive security, understanding binary code is crucial for exploiting vulnerabilities, developing sophisticated malware~\cite{mohan2012frankenstein}, and advancing penetration testing techniques~\cite{szekeres2013sok}. Yet, to be genuinely transformative in these realms, a deep, semantic understanding of binary code is vital---one that extends beyond mere pattern recognition and delves into the embedded logic, intent, and function. \looseness=-1
%However, achieving groundbreaking innovations necessitates more than superficial pattern identification; it demands an in-depth, semantic insight into the binary code, unraveling the intertwined threads of logic, intention, and functionality. 


%Code comments are crucial in software development as they provide explanations and context about the code, making it easier for other developers to understand and maintain the codebase. They also serve as documentation, helping developers, including the original author, to remember the purpose and functionality of different code sections, reducing errors and speeding up debugging and maintenance.

The recent surge in computational capabilities, primarily due to the advent of ``large language models'' (LLMs) like ChatGPT and GPT-4, offers a potential avenue to address these complexities. These innovative models represent significant strides towards realizing the ambitions of strong artificial intelligence, boasting capabilities that enable interactions mirroring human-like intelligence and understanding. The potentialities of LLMs like ChatGPT have already sparked discussions about revolutionary shifts in software engineering and source code analysis based tasks (e.g., Fuzzing~\cite{}, repair~\cite{}), painting a picture of a future where software development and analysis are profoundly shaped by advanced language models.
\Xin{ChatGPT has exhibited promising capacities in software engineering. Cite the papers.}



However, the journey to harness the full potential of LLMs in binary code analysis is far from straightforward. These models, developed by OpenAI, are predominantly trained on publicly accessible data, including massive amount of textual content and code repositories. A notable and critical void in their training data is the sparse presence of binary code, raising significant questions about their proficiency in deciphering binary code semantics. This scarcity of binary code in training data potentially caps the models' comprehension abilities in binary code analysis, leaving a vital area in software engineering largely untouched and brimming with unexplored potentials. The unexplored territory between LLMs and binary code analysis necessitates an exploration aimed at revealing the extent to which models like GPT-4 and ChatGPT can navigate the intricacies of binary code.


Addressing the aforementioned limitations and uncertainties, this paper proposes a systematic exploration of GPT-4’s and ChatGPT’s abilities to understand binary code. The endeavor is fraught with challenges, owing to the nuances of binary code and the gaps in the training data of current LLMs. The exploration strives not only to bring clarity to the capabilities of these advanced models in binary code analysis but also to spotlight innovative methodologies and approaches that could potentially amplify their effectiveness in this domain. This measurement investigation is geared towards uncovering deeper insights and paving the way for leveraging LLMs in binary code analysis, possibly unlocking new paradigms in software engineering and security.


Our comprehensive experiments and analyses bring to the fore nuanced insights and a clearer understanding of the capabilities and limitations of LLMs in binary code analysis. The outcomes of this study are multifaceted, highlighting promising aspects and pinpointing areas necessitating further refinement and research. We delve into how models like GPT-4 and ChatGPT, despite their groundbreaking generalization abilities, encounter unique challenges when applied to binary code, offering a detailed exposition of their performance and the possible enhancements needed. The findings from this study serve as a beacon, illuminating the path forward in the convergence of large language models and binary code analysis, and provide a foundation upon which future innovations can build, potentially reshaping the landscape of binary code analysis and software engineering.

\paragraph{Contributions} This paper makes the following key contributions.

\begin{packeditemize}
    

    \item \textbf{Unprecedented Exploration and Analytical Depth:}
    We conduct a groundbreaking exploration and in-depth analysis of the potentials of Large Language Models (LLMs), particularly GPT-4 and ChatGPT, in binary code analysis, revealing the complexities and offering insights into this novel and intricate domain.
    
    \item \textbf{Methodological Innovation and Empirical Insights:}
    We pioneer innovative methodologies and conduct rigorous empirical evaluations to understand and enhance the applicability of LLMs in binary code. Our findings provide nuanced insights into the strengths and limitations, suggesting practical enhancements to leverage LLMs effectively in software engineering and computer security.
    
    \item \textbf{Comprehensive Framework and Practical Implications:}
    Our work establishes a comprehensive framework for understanding the interplay between LLMs and binary code analysis, offering detailed implications and serving as a foundational reference for future theoretical and practical endeavors in diverse application areas, including software development and defensive security.
\end{packeditemize} 


\ignore{
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%These models, known for their unprecedented versatility in various domains, promise to be potential game-changers for binary code analysis. Their achievements in fields like natural language processing provide a tantalizing hint of their potential; however, the specific nuances of binary code understanding via these models remain largely unexplored.
%The advent of Large Language Models (LLMs) like ChatGPT and GPT-4 is a landmark development in the field of artificial intelligence, garnering widespread attention, particularly among those engaged in binary reverse engineering. These innovative models represent significant strides towards realizing the ambitions of strong artificial intelligence, boasting capabilities that enable interactions mirroring human-like intelligence and understanding. The potentialities of LLMs like ChatGPT have already sparked discussions about revolutionary shifts in software engineering, painting a picture of a future where software development and analysis are profoundly shaped by advanced language models.



%These tools have shown great promise in understanding and generating human language. Could they also help us better understand binary code? Especially when considering that these models aren't explicitly trained on a lot of binary code data.

%%The integration of scale and attention-based architectures has led to the development of language models with an extraordinary level of versatility. These models, known as ``large language models'' (LLMs), have demonstrated remarkable and sometimes even superhuman abilities across various tasks, including zero-shot and few-shot scenarios. While their generality is impressive, it raises the question of control: how can we harness the immense power of LLMs to decipher the semantics of binary code through reverse engineering?

% The introduction of generative large language models, such as ChatGPT, has already spurred fervent discussion from security professionals, ranging from fear that malware developers could use these AI tools to develop the more advanced malware, to excitement about the new types of opportunities that reverse engineers might leverage to help understand binary code.  
% However, given the nascent nature of these tools, we currently lack fundamental knowledge related to
% how well they perform in different security settings, and the
% potential promise (or danger) that they might pose to traditional
% forms of reverse engineering.

%%The advent of powerful language models like ChatGPT has sparked intense debates among security experts. On one hand, there are concerns about the possibility of malicious actors utilizing AI tools to create more sophisticated malware. On the other hand, there is excitement surrounding the potential for reverse engineers to leverage these tools in novel ways to comprehend binary code. Nevertheless, due to the relative newness of these technologies, we still lack essential understanding regarding their performance in various security environments. Moreover, we remain uncertain about the potential benefits or risks they might introduce to conventional reverse engineering practices.

% GPT-4 and ChatGPT, the recently introduced generative large language models, have attracted significant attention within the binary reverse engineering community due to its reported capacities in the longstanding dream of strong artificial intelligence: to interact with users like human beings with exhibiting the dramatic intelligence.
% Reported results have suggested that OpenAI models, e.g., ChatGPT will be transformative for the field of software engineering, and that LLM-driven software engineering has a bright future.
% However, the application of GPT-4 and ChatGPT in binary code understanding remains unexplored. 
% OpenAI models are trained with public corpus, including online textual data and code repositories.
% However, such data may rarely contain the binary code data, which may limits their abilities in binary code understanding.
% For this, we propose to investigate the binary code understanding capacity of GPT-4 and ChatGPT in binary code understanding.

The recent introduction of ChatGPT and GPT-4, powerful generative language models, has generated significant interest within the binary reverse engineering community. These models have been hailed as a major step towards achieving the long-desired goal of strong artificial intelligence, enabling human-like interactions and showcasing impressive intelligence capabilities.
Initial reports have suggested that OpenAI models, including ChatGPT, have the potential to revolutionize the field of software engineering, signaling a promising future for LLM-driven software engineering.
However, the specific application of GPT-4 and ChatGPT in the realm of binary code understanding remains largely unexplored. These OpenAI models are trained on publicly available data sources, encompassing online textual data and code repositories. Unfortunately, binary code data is rarely present in such sources, which may limit the models' abilities in comprehending binary code.
To address this limitation, we propose an investigation into the binary code understanding capacity of GPT-4 and ChatGPT. By exploring their capabilities in this domain, we aim to shed light on their potential in enhancing binary code analysis and comprehension.

Inspired by the success of LLMs in the fields of source code summarization and natural language processing (NLP), we aim to study the effectiveness of existing LLMs in comprehending the semantics of binary code. 
This area of investigation, to the best of our knowledge, has not yet been explored.
}

==> sections/overview.tex <==



\subsection{Challenges}
\label{sec:challenge}

% \paragraph{Effective Prompt Design}
\paragraph{C1: Task Adaption of LLMs}
Generative LLMs, such as ChatGPT and Llama, are pretrained in general English corpora with a small proportion of source code datasets~\cite{touvron2023llama}, aimed mainly at natural language tasks.
Adapting LLMs to our tasks requires mitigating the semantic gap between pre-training tasks and our binary code summarization task.
% Existing finetuning based solutions for domain adaption cannot fit our needs because they require model weight access, which is not accessible for closed-source LLMs such as ChatGPT, a prohibitively large binary summarization dataset, and expensive computational resources~\cite{liu2023pre}.
% Large language models are block-box which makes it hard to determine the best prompts for our binary code summarization task.
% Prompts play the important roles in directing LLMs to generate effective response.
% The design of effective prompts can help ensure that LLMs provide results that comply with predetermined standards or requirements.
While directly finetuning LLMs on our tasks is extremely challenging as discussed in \S\ref{sec:backgound}, formulation of well-crafted prompts is a promising solution, which is instrumental in ensuring that LLMs yield outputs that align with our task-specific needs.
% Users can direct the language model to generate desired responses by giving clear instructions through prompts. This degree of oversight can aid in ensuring that AI models provide results that comply with predetermined standards or requirements.
%Large language models have shown the promissing results in many machine learning tasks, e.g., natural langauge understanding and information retrieval.
% Moreover, how prompts work effectively is still non-interpretable for human beings due to its deep network architectures and nonlinearity.
% However, LLMs are 
Meanwhile, it has been found that instructing LLMs with varied directives can yield distinct performance outcomes in natural language processing tasks \cite{zhou2022large}.
In the context of summarizing binary code with LLMs, devising effective prompts remains a paramount concern.
% However, it's found that prompting LLMs with different instructions can result in different performance in NLP tasks~\cite{zhou2022large}, designing the effective prompts is a very important task for binary code summarization.
However, the black-box nature of LLMs makes it hard to determine the best prompts for our binary code summarization task.
That said, it's hard to interpret what input words or features contribute the most for results generated by large langauge models though there have been efforts to explain LLMs~\cite{liu2023pre}.
The problem is even harder for the closed-source LLMs, e.g., GPT-4 and ChatGPT, whose model architectures and weights are not accessible for us.
%Altough there have been efforts in prompting LLMs for tasks that are similar to us, e.g., source code summarization, we argue that 
% Therefore, there is a need for designing the effective prompts to maximize the performance of LLMs.

\paragraph{C2: Lack of large-scale and comprehensive dataset}
For our binary code summarization tasks, there is no large-scale dataset with ground truth, which covers the various real-world binaries that are compiled with various compilation settings.
The commercial off-the-shelf (COTS) binaries are compiled with different compilation settings, e.g., computer architectures (e.g., x64, x86 and ARM) and optimization levels (e.g., O0, O1 and O2).
Compiling source projects with different compilation settings results in diverse binaries from different aspects.
For example, different computer architectures generate code with different instruction sets, which are the different vocabularies for machine learning models.
Moreover, it has been found that the higher optimization levels result in binary functions with more semantic information because the callee can be inlined into callers~\cite{jin2022symlm}.
In addition to the diverse binaries, ground-truth summaries of binary code are also necessary because we cannot evaluate the LLM-generated summaries without such gold references.
However, the binaries do not carry such semantic summaries and the symbol names, such as function names, cannot represent the complete code semantics though they are usually stripped in COTS binaries.
% For example, Figure \xy presents the assembly code of binaries compiled with different computer architecture and Figure \xy presents the decompiled code compiled from binaries with different optimization levels.
% The different computer architectures generate code with different instruction sets, which are the different vocabularies for machine learning models.
% Function inlining has been shown to be popular for binaries compiled with higher optimization levels~\cite{jin2022symlm}. 
% Moreover, the dataset should comprehensively cover the diverse binaries compiled from various compilation settings.
% Last but not least, this dataset should include ground truth descriptions to truly represent binary code semantics. 
%To obtain the profound insights of LLMs, we need to have large-scale experiments on existing LLMs.
% This is necessary because commercial off-the-shelf (COTS) binaries are compiled with different compilation settings, i.e., compilers (e.g., GCC and Clang), computer architectures (e.g., x64, x86 and ARM), and optimization levels (e.g., O0, O1 and O2).
% Compiling source projects with different compilation settings results in diverse binaries.
% For example, Figure \xy presents the assembly code of binaries compiled with different computer architecture and Figure \xy presents the decompiled code compiled from binaries with different optimization levels.
% The different computer architectures generate code with different instruction sets, which are the different vocabularies for machine learning models.
% Function inlining has been shown to be popular for binaries compiled with higher optimization levels~\cite{jin2022symlm}. 
Therefore, the large-scale and comprehensive binary dataset with ground-truth code summaries is necessary for us to obtain profound insights.
%\paragraph{Semantic gap between pre-training and downstream task} Large language models (LLMs), such as OpenAI GPT-4 and ChatGPT are pre-trained on a very large corpus of text and source code, which is semantically different from binary code, e.g., binary raw bytes, assembly code, and decompiler-generated code.
%Moreover, there are gaps between the pre-training and fine-tuning processes of LLMs.
%For LLMs from the BERT and T5 families, they are generally pre-trained using the masked language modeling (MLM) objective. During pretraining, random tokens are masked in input sentences and LLMs learn to predict these masked tokens based on the surrounding context. 
%For OpenAI models, such as GPT-2, they are pre-trained using an autoregressive language modeling objective, which predicts the next words in a sequence conditioned on the previous words. This approach allows LLMs to generate coherent and contextually appropriate text.
%However, when leveraging these LLMs to summarize binary code, the input involves only binary code, e.g., binary raw bytes. For the LLMs in the BERT family, the learning objective changes to a cross-modal generation task.
%The disparity in inputs and objectives during pretraining and fine-tuning makes it challenging to fully leverage the knowledge contained within pretrained models. As a result, this often leads to suboptimal results in downstream tasks.

\paragraph{C3: Various Binary Code Representations} 
Binary code are stored as raw bytes in the binary files.
To assist the various binary analysis tasks, binary code is processed into different representations, e.g., assembly code, intermediate representation  (IR) code, and decompiled code.
For example, the BAP-IR code was used to predict symbol names of stripped binaries due to the Static Single Assignment (SSA) representation that assigns a unique name to each variable in the code, ensuring that each variable is assigned only a value once~\cite{he2018debin}.
However, it is not clear which binary code representations can optimize the code comprehension capacities of LLMs.
% While binary code can be represented as machine code, assembly code, intermediate representations, decompiled code, it's hard to determine the best representations for our binary code understanding tasks.
% Binary code are stored as raw bytes in binary executable files.
% To reverse engineer binary code semantics, security professionals usually use disassemblers and decompilers to generate low-level code representations, i.e., assembly code and decompiled code. 
% In addition, reverse engineers also consider to generate intermediate representations (IR) for binaries.
% The benefits for IR analysis is the Static Single Assignment (SSA) representation that assigns a unique name to each variable in the code, ensuring that each variable is only assigned a value once.
% The use of SSA form has several benefits in program analysis and optimization. It simplifies many compiler optimizations by making it easier to reason about the program's control flow and data dependencies. SSA form allows for better dead code elimination, constant propagation, and register allocation, among other optimizations.
When faced with so many binary code representations, existing LLM-based binary reverse engineering frameworks design binary-specific neural architectures without exploring the best representations for LLMs.
For example, varBERT~\cite{banerjee2021variable} takes as input raw decompiler output, i.e., decompiled code to infer variable types.
SymLM~\cite{jin2022symlm} uses the disassembler output, that is, the assembly code, to predict function names.
% For us, it is not clear which binary code representation is better for binary code summarization.
Without any systematic investigation of suitable binary inputs to LLMs, it is challenging to optimize the performance of LLMs in our task. 

%\paragraph{Diverse Binaries Compiled from Various Compilation Settings}


\paragraph{C4: Evaluation of Fuzzy Code Summaries}
Our objective is to generate human-readable code summaries by LLMs.
LLM outputs are in human languages, which convey semantic meanings in a fuzzy manner.
That is, the code summaries generated by LLMs can express the same semantics with syntactically different words, phrases, and sentences, which may contain acronyms, synonyms, and even misspellings.
% There is the need to design an effective measurement metrics that can capture the correct semantics considering binary code summaries are noisy natural languages.
% Natural languages are noisy so that the same semantic meanings can be expressed with different words and phrases.
While facing such noisy code summaries, heuristic evaluation metrics, such as word matching, will fail to measure the true performance of LLMs.
Although there have been efforts to solve this problem in similar tasks as ours, i.e., function name prediction, their word cluster based solution cannot be applied to binary code summarization because the summaries are in sentences that are much longer and more complicated than the short function names. \looseness=-1

\subsection{Insights and Solutions}
\label{sec:solutions}

\paragraph{S1: In-context Prompt Synthesis and Optimization}
% To adapt LLMs to our binary summarization task, prompts that are manually-crafted by experienced binary reverse engineers or prompt engineering experts may yield good performance of LLMs.
% It cannot optimize the performance of LLMs as the prompt generation process is subjective.
% Instead of adopting manually generated prompts, we propose in-context prompt synthesis and optimization methods to address this problem based on two observations.
% First, it has been found that LLMs are human-level prompt engineers.
% Therefore, we can search over a pool of prompt candidates synthesized by LLMs.
% Next, we found that LLMs can self-improve which means we can optimize the LLM-generated prompts to yield the optimal LLMs.
% Finally, we perform in-context prompt evaluations to opt the best prompt for our task.
To adapt LLMs for our binary summarization task, the creation of prompts crafted by experienced binary reverse engineers or prompt engineering professionals may yield commendable LLM performance. 
Nevertheless, this approach is constrained by its subjectivity and may not fully optimize LLM performance.
Instead relying solely on manually generated prompts, we propose a novel approach involving in-context prompt synthesis and optimization techniques, grounded in two key observations. 
Firstly, LLMs have demonstrated a capacity akin to that of human prompt engineers~\cite{zhou2022large}. 
Therefore, we can search over a pool of prompt candidates synthesized by both human beings and LLMs themselves. 
Secondly, LLMs exhibit the ability to self-improve~\cite{huang2022large}, which implies that we can optimize the prompts generated by LLMs to attain optimal performance. 
Finally, we undertake in-context prompt evaluations on the binary code summarization dataset to select the most suitable prompt candidates.
% In order to address the semantic gap between pretraining and the downstream binary code summarization task, a common approach is to fine-tune language models (LLMs) using domain-specific datasets. This typically involves employing parameter-efficient fine-tuning methods, where the majority of the LLM's parameters are kept frozen and only a small number of task-specific parameters are adjusted.
% However, performing full-model fine-tuning requires a prohibitively large data set, and it can be computationally expensive, especially on consumer-grade hardware, making it challenging to provide greater accessibility in LLM research and deployment.
% Prompt tuning is introduced as a solution to overcome resource limitations associated with traditional fine-tuning methods. For example, when summarizing binary code, prompt tuning involves constructing the input by combining a contextual instruction, such as ``You are a helpful AI assistant trained to understand binary code'', with a natural language prompt. This allows the language models to capture the semantics of the binary code.
% For BERT-family language models, prompt tuning involves crafting the prompt to simulate the mask token prediction process. This can be achieved by adding a prompt like ``This binary function is assigned to [MASK]''. By incorporating these prompts, the models gain a better understanding of the context and generate more accurate summaries of the binary code.
% [TODO] Introduce how we use in-context learning

\paragraph{S2: Comment-enabled Comprehensive and Extensive Dataset Construction}
\Xin{Cite source code summarization works to motivate why code comments can be used as summaries. There are multiple ways to represent the code semantics. The common practice}
Compared to binary code, source code carries far richer semantic information, e.g., variable and function names, thus existing source code models have exhibited promising performance on code summarization.
To obtain code summary references for binary code, an intuitive approach is to generate code summaries using existing source code summarization models and systems, e.g., Github Copilot~\cite{chen2021evaluating}, and then label binary code with generated summaries.
However, such artificial code summaries can contain errors and carry model-specific features~\cite{shi2022evaluation}.
While facing the challenge of obtaining summary references, we observe that developers can write comments to document the functionality of production code in different levels.
Therefore, we use such comments as the gold reference by matching the function-level source code comments to binary functions.
Specifically, we first curate open-source projects and then parse function comments in source files.
Next, we compile them into binaries with different compilation settings to generate diverse binaries.
Finally, we map the extracted function comments with binary functions.
To this end, we generate a large-scale and comprehensive binary summary dataset with developer-written comments as ground truth.

\paragraph{S3: Comprehensive Evaluations on Binary Code Representations}
While binary code can be represented in different formats, we conduct a large-scale study directly on these representations at the function level.
% First, we compile 
Specifically, we first generate the different binary code representations by (\textit{i}) extracting raw bytes of binary functions, (\textit{ii}) disassembling binaries into assembly code,  (\textit{iii}) generating IR code of binaries, and (\textit{iv}) decompiling binaries into decompiled code.
Next, we perform large-scale evaluations on these code representations to study LLMs' capacities of comprehending them. \ZQ{This may be too trivial, and no need to mention}

\paragraph{S4: Semantic Evaluation of LLM-generated Summaries}
While facing the similar issue of evaluating fuzzy code summaries, the source code summarization community borrow the evaluation methods of neural machine translation, e.g., BLEU~\cite{papineni2002bleu}, METEOR~\cite{banerjee2005meteor}, and ROUGE~\cite{lin2004rouge}.
BLEU score is computed by matching the n-grams that coexist in both summary reference and generated summary candidate. 
It has been widely used for its ease of understanding and cost-effective calculation, it has inherent limitations. 
% One of the major issues is that not all words in a sentence are equally important, and many words have close synonyms. 
% For instance, changing the word ``maximum'' to ``minimum'' from the summary sentence can drastically alter its meaning, while replacing ``decrease'' with 'reduce' may not have such a significant impact. 
As discussed in challenge \textbf{C4}, abbreviations, misspellings, and semantic similar phrases are widely used in code summaries.
Unfortunately, BLEU and the other exact-matching metrics, e.g., METEOR and ROUGE, fail to capture semantic meanings.
In this paper, we propose to measure the LLM-generaed binary code summaries by their semantics.
Specifically, we first generate semantic embeddings of both the summary references and the generated summary candidates.
Next, we calculate the semantic similarity of the embeddings, and the similarity scores serve as the evaluation metrics for our study.

\subsection{Overview}
\label{sec:overview}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figures/system-workflow-v1.pdf}
    \caption{Study Workflow. 
    % \Xin{Remove Pretraining}
    We first construct a binary code summarization dataset, including binaries compiled from open-source repositories across four computer architectures and optimization levels along with various code representations. Next, prompts are synthesized and optimized using LLMs, and the best prompts are selected through evaluation. The last step includes online testing on ous target LLMs and semantic evaluation, where binary code summaries are converted into semantic embeddings to assess LLMs' understanding of binary code. 
    % \Xin{Fix numbers and position of prompt optimization}
    }
    \label{fig:sys-workflow}
\end{figure*}

\autoref{fig:sys-workflow} presents the workflow of our study, which includes three key steps. 
We first construct a large-scale and comprehensive binary code summarization dataset by compiling open-source repositories into diverse binaries across four computer architectures (i.e., x86, x64, ARM, and MIPS) and four optimization levels (i.e., O0-O3).
These binaries are fed into our binary analyzers to generate code representations, including decompiled code, IR code, assembly code, and raw bytes, along with source code.
Note that we have decompiled binaries using three popular decompilers, covering Ghidra, the open-source decompiler, Hex-rays, commercial decompiler, and Angr, the fast-developing decompiler.
Next, we generate a pool of prompts by leveraging LLMs to synthesize initial prompts and variants that are further optimized by LLMs along with human-generated prompts.
The best-suite prompts are selected by in-context evaluation on binary code summarization dataset.
The third step involves both online testing and semantic evaluation of test-generated prompts.
For testing, we feed our target LLMs, i.e., ChatGPT, GPT-4, Llama 2, and Code Llama, with our extensive binary summarization test samples embedded in the selected prompts.
The generated binary code summaries are encoded into semantic embeddings by a pretrained LLM-based summary encoder.
The embeddings are further computed as semantic similarity scores, which reveal LLMs' capacities in binary code comprehension.
% \ZQ{I feel it's hard to call the system BinGPT, as we are not inventing any new GPT, and instead we just measure}

% \Xin{Swap prompt synthesis and binary dataset construction}

\paragraph{Study Scope} In this paper, we focus on the binary code summarization at the function level.
% Our design choice is based on the  observations.
Functions are the building blocks in both source code and binary code, and it's easier to identify and map developer-written code comments from source functions to binary functions compared to the lower- and higher-level code snippets, e.g., code blocks.
Moreover, we target the generative LLMs, including ChatGPT, GPT-4, Llama 2 and Code Llama.
Our design choice is based on the observation that such LLMs have exhibited impressive generalizability and superior performance in both natural language processing and code comprehension tasks, e.g., source code summarization and code generation tasks~\cite{ma2023scope}.
For evaluating binary code summarization, LLMs are given raw-bytes, assembly code, intermediate representation (IR), and decompiled code as the representations of binary functions.
% \Xin{Specify what the target for this paper is. We study the }



==> tables/src-projects.tex <==
\begin{table}[]
\centering
% \small
\caption{The Projects in Our Dataset\Xin{Emphrasize the project size much larger than existing works. Show \# of line codes. Focus on code complexity. Number of functions.}}
% \vspace{-0.1in}
\begin{tabular}{l|r||l|r}
\toprule
\textbf{Project} & \textbf{Version} & \textbf{Project} & \textbf{Version} \\ \midrule
coreutils        & 8.32                                 & mpfr             & 4.0.2            \\
findutils        & 4.9.0            & curl             & 7.86.0           \\
wget2            & 2.0.1            & libiconv         & 1.17                                 \\
mailutils        & 3.8                                  & units            & 2.22                                 \\
autoconf         & 2.71                                 & readline         & 8.2                                  \\
nettle           & 3.8                                  & inetutils        & 2.4                                  \\
bison            & 3.8                                  & adns             & 1.6.0            \\
lightning        & 2.2.0            & datamash         & 1.8                                  \\
bash             & 5.2                                  & ncurses          & 6.3                                  \\
dico             & 2.11                                 & libunistring     & 1.0                                  \\
sed              & 4.9                                  & nano             & 7.0                                  \\
less             & 608                                  & libpng           & 1.6.39           \\
libtool          & 2.4.7            & libidn2          & 2.3.4            \\
diffutils        & 3.8                                  & gmp              & 6.2.1           \\
gama             & 2.05                                 & gettext          & 0.21                                 \\
gawk             & 5.2.1            & grep             & 3.8                                  \\
cflow            & 1.7            & gzip             & 1.12                                 \\
gss              & 1.0.4            & freeipmi         & 1.6.10           \\
openssl          & 3.0.6            & libredwg         & 0.12                                 \\
tar              & 1.34                                 & texinfo          & 7.0                                    \\
binutils         & 2.39                                 & poke             & 2.4                                  \\
libmicrohttpd    & 0.9.75           & direvent         & 5.2                                  \\
% cflow            & 1.7                                  &    -              &  - \\
\bottomrule
\end{tabular}
\label{tab:source-projects}
\end{table}
